On Meritocracy in Optimal Set Selection

Typically, merit is defined with respect to some intrinsic measure of worth. We instead consider a setting where an individual's worth is \emph{relative}: when a Decision Maker (DM) selects a set of individuals from a population to maximise expected utility, it is natural to consider the \emph{Expected Marginal Contribution} (EMC) of each person to the utility. We show that this notion satisfies an axiomatic definition of fairness for this setting. We also show that for certain policy structures, this notion of fairness is aligned with maximising expected utility, while for linear utility functions it is identical to the Shapley value. However, for certain natural policies, such as those that select individuals with a specific set of attributes (e.g. high enough test scores for college admissions), there is a trade-off between meritocracy and utility maximisation. We analyse the effect of constraints on the policy on both utility and fairness in extensive experiments based on college admissions and outcomes in Norwegian universities.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> macros.tex <==
%%Macros and packages
\usepackage[utf8]{inputenc}
\usepackage{fontenc} %for xelatex of lualatex
\usepackage{hyperref}       % hyperlinks [pdfborder={0 0 0}] to remove bad looking colored boxes
\usepackage{url}            % simple URL typesetting
% \usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}
\usepackage{enumitem}%\setlist{nolistsep}
\usepackage{isomath}
% For figures
\usepackage{graphicx,subcaption}%,epstopdf}
\usepackage{grffile}
\usepackage{pdfpages} 

%For figures
\usepackage{caption}

% for professional tables
\usepackage{booktabs} 
% for maths notations
\usepackage{mathtools,amsmath,amssymb,amsfonts,amsthm,dsfont}
% \usepackage{mathtools,amsmath,amsfonts,amsthm,dsfont}

% for algorithm
\usepackage{algorithm}
\usepackage{algpseudocode}% For bibliography
%\usepackage[sort&compress]{natbib}
%\usepackage{natbibspacing}
% For Mathematical figures and networks
\usepackage{tikz}
\usetikzlibrary{bayesnet,arrows}
% for appendix proofs
%\usepackage{natbib,bibunits}
%\usepackage{environ,etoolbox}
%\usepackage[bibliography=common]{apxproof}
% hyperref makes hyperlinks in the resulting PDF.
%\usepackage[pdfborder={0 0 0}]{hyperref}

\usepackage[nameinlink,sort&compress]{cleveref}
\crefname{construction}{Construction}{Constructions}
\crefname{claim}{Claim}{Claims}
\crefname{paragraph}{Paragraph}{Paragraphs}
\crefname{observation}{Observation}{Observations}
\crefname{theorem}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmata}
\crefname{proposition}{Proposition}{Propositions}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{remark}{Remark}{Remarks}
\crefname{section}{Section}{sections}
\crefname{chapter}{Chapter}{Chapters}
\crefname{figure}{Figure}{Figures}
\crefname{table}{Table}{Tables}
\crefname{definition}{Definition}{Definitions}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{equation}{Equation}{Equations}
\crefname{appendix}{Appendix}{Appendices}

%For affiliations
%\usepackage{authblk}
\newcommand{\footremember}[2]{%
    \footnote{#2}
    \newcounter{#1}
    \setcounter{#1}{\value{footnote}}%
}
\newcommand{\footrecall}[1]{%
    \footnotemark[\value{#1}]%
} 



% Attempt to make hyperref and algorithmic work together better:
%\newcommand{\theHalgorithm}{\arabic{algorithm}}
%%New theorem environments
\newtheorem{theorem}{Theorem}
\makeatletter
\newenvironment{sublemma}[1]{%
  \def\sublemmacounter{#1}%
  \refstepcounter{#1}%
  \protected@edef\theparentnumber{\csname the#1\endcsname}%
  \setcounter{parentnumber}{\value{#1}}%
  \setcounter{#1}{0}%
  \expandafter\def\csname the#1\endcsname{\theparentnumber \alph{#1}}%
  % To keep hyperref happy, update H-counter as well
  \expandafter\def\csname theH#1\endcsname{lemma.\theparentnumber \alph{#1}}%
  \unskip\ignorespaces
}{%
  \setcounter{\sublemmacounter}{\value{parentnumber}}%
  \ignorespacesafterend
}
\makeatother
\newcounter{parentnumber}
\newtheorem{lemma}{Lemma}
\newtheorem{fact}{Fact}
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{assumption}{Assumption}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem{conjecture}{Conjecture}
\theoremstyle{definition}
\newtheorem{definition}{Definition}


% \newtheorem{todo}{To-do}

%\usepackage{algpseudocode}
%% Tikz macros
\tikzstyle{privplate} = [draw, rectangle, dashed, fit=#1]
\tikzstyle{privplate caption} = [caption, node distance=0, inner sep=0pt,
above left=10pt and 0pt of #1.north east]
\newcommand{\privplate}[4][]{ %
	\node[wrap=#3] (#2-wrap) {}; %
	\node[privplate caption=#2-wrap] (#2-caption) {#4}; %
	\node[privplate=(#2-wrap)(#2-caption), #1] (#2) {};% %
}
\tikzstyle{decision} = [rectangle, text centered, minimum width=2em, minimum height=2em, draw=black]
% \| is used only inside KL-divergence, should add space
\let\olddbar\|
\renewcommand{\|}{\,{\olddbar}\,}
%%Notations
\newcommand{\val}{v}
% \newcommand{\shapley}{v^{\textrm{S}}}
\newcommand{\util}{U}
\newcommand{\param}{\vectorsym{\boldsymbol{\theta}}}
\newcommand{\Param}{\Theta}
\newcommand{\vparam}{\vectorsym{\boldsymbol{\theta}}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\reg}{\mathrm{Reg}}
\newcommand{\alg}{\mathcal{A}}
\newcommand{\mech}{\mathcal{M}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\br}{\vectorsym{r}}
\newcommand{\BR}{\vectorsym{R}}
\newcommand{\CX}{\mathcal{X}}
\newcommand{\CY}{\mathcal{Y}}
\newcommand{\BZ}{\vectorsym{Z}}
\newcommand{\bz}{\vectorsym{z}}
\newcommand{\bp}{\vectorsym{p}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bct}{\mathbf{b}}
\newcommand{\predictor}{\mathbf{f}}
\newcommand{\EMC}{\Delta}
\newcommand{\indiv}{j}
\newcommand{\egpol}{\pol_{\text{egal}}}
\newcommand{\ut}{u}
\newcommand{\Beta}{\textrm{Beta}}
\newcommand{\Multinomial}{\textrm{Multinomial}}
\newcommand{\Softmax}{\textrm{Softmax}}
\newcommand{\Bernoulli}{\textrm{Bernoulli}}
\def\kldiv#1#2{D\left( #1 \| #2\right)}
\def\abs#1{\left| #1 \right|}
\def\recip#1{\frac{1}{#1}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand \bias {\textit{bias}}
\newcommand \noise {\textit{noise}}
\newcommand \male {\mathrm{male}}
\newcommand \female {\mathrm{female}}
\newcommand \gender {\mathrm{gen}}
\newcommand \sk {\mathrm{sk}}
\newcommand \gpa {\mathrm{gpa}}
\newcommand \tal {\mathrm{tal}}

\newcommand \pol {\ensuremath{\pi}}
\newcommand \Pol {\ensuremath{\Pi}}
\newcommand \model {\ensuremath{\nu}}
\newcommand \bel {\ensuremath{\beta}}
\newcommand \qual {\ensuremath{q}}
\newcommand \feat {\ensuremath{\phi}}
\newcommand \act {\mathbf{a}} % {\vectorsym{a}} %{\ensuremath{\vectorsym{a}}}
\newcommand \acti {\mathbf{a}_i} % {\ensuremath{a}_i}
\newcommand \actj {\mathbf{a}_j} % {\ensuremath{a}_j}
\newcommand \Act {\ensuremath{\mathcal{A}}}
\newcommand \Hist {\ensuremath{\mathcal{H}}}
\newcommand \hist {\ensuremath{H}}
\newcommand \dist {\ensuremath{\vectorsym{\Delta}}}
%\newcommand \Gen {\ensuremath{\mathcal{G}}}
\newcommand \gen {\ensuremath{\mathcal{G}}}
\newcommand \generator {\ensuremath{\theta}}
\newcommand \defn {\mathrel{\triangleq}}
\newcommand \dd {\,\mathrm{d}}
\newcommand{\game}{\mathcal{G}}
\newcommand{\pop}{\mathcal{N}}
\newcommand{\nPop}{N}
\newcommand \dataset {\ensuremath{\mathcal{D}}}
\newcommand \sensitive {\ensuremath{\mathcal{S}}}
\newcommand \outcome {\ensuremath{\mathcal{Y}}}
\newcommand{\cost}{\ensuremath{c}}
\newcommand{\imputation}{\ensuremath{\phi}}
\newcommand{\reward}{\ensuremath{\mathcal{R}}}
\newcommand{\coalition}{\ensuremath{\mathcal{C}}}
\newcommand{\distr}{\xi}
\newcommand{\contr}[2]{\Delta_{#1} \util ({#2} } %#1 = individual, #2 = policy
\DeclareMathOperator{\res}{Res}
%\newcommand{\res}{Res}
\DeclareMathOperator{\diversity}{Div}
\renewcommand{\colon}{\, : \,}
\newif\ifnotes
\newif\iflongversion
\newif\ifshortversion
\newif\ifpreprint



\newcommand\set[1] {\left\lbrace #1 \right\rbrace}
\newcommand\ind[1] {\mathbb{I}\left\lbrace #1 \right\rbrace}
\newcommand\cset[2] {\left\{#1 ~\middle|~ #2\right\}}

%\newcommand\gen{\ensuremath{\mathcal{G}}}
\newcommand\Simplex {{\mathcal P}}
\newcommand\Reals {{\mathds{R}}}
\newcommand\Naturals {{\mathds{N}}} 

% For Deviation from Meritocracy
\newcommand{\devswap}{\text{Dev}_\text{swap}}
\newcommand{\devchange}{\text{Dev}_\text{local}}


\tikzstyle{place}=[circle,draw=black,inner sep=0mm, minimum size=6mm]

\tikzstyle{utility}=[diamond,draw=black,draw=blue!50,fill=blue!10,inner sep=0mm, minimum size=8mm]
\tikzstyle{select}=[rectangle,draw=black,draw=blue!50,fill=blue!10,inner sep=0mm, minimum size=6mm]
\tikzstyle{hidden}=[dashed,draw=black,fill=red!10]
\tikzstyle{RV}=[circle,draw=black,draw=blue!50,fill=blue!10,inner sep=0mm, minimum size=6mm]

\tikzstyle{transition}=[rectangle,draw=black!50,fill=black!20,thick]
\tikzstyle{someset}=[circle,draw=black,minimum size=8mm]
\tikzstyle{point}=[circle,draw=black,fill=black]


%% Appendix
%\renewcommand{\appendixsectionformat}[2]{Supplementary Material for Section #1 (#2)}

%%Editing
\newcommand{\cdcomment}[1]{[CD: \textcolor{red}{#1}]}
\newcommand{\dbcomment}[1]{[DB: \textcolor{blue}{#1}]}
\newcommand{\amgcomment}[1]{[AMG: \textcolor{blue!60!green!60}{#1}]}
\newcommand{\mscomment}[1]{[MS: \textcolor{purple}{#1}]}
\newcommand{\response}[1]{\textcolor{purple}{#1}}




\DeclareMathOperator{\emc}{EMC}
\DeclareMathOperator{\shapley}{Shapley}

==> sections/EMC_and_meritocracy2.tex <==
\section{Expected marginal contributions and meritocracy}\label{sec:EMC and Meritocracy}

% While maximising utility is appropriate for a society, e.g., if the utility reflects social welfare, it is not necessarily meritocratic. 
In order to define and analyse meritocracy in our setting, we first define the expected marginal contribution of an individual (given a policy) in \cref{sec:exp_marg_contr}.
% For certain policy structures, this is a linear transformation of the expected utility with respect to the policy parameters. In consequence, at any local maximum, the gradient and so the expected marginal contribution is zero. This can be interpreted as saying that the utility, i.e., the social welfare, would be reduced by changing the current allocation. 
We then base our definition of meritocracy on two crucial properties linked to the expected marginal contribution of individuals in \cref{sec: meritocracy}.



\subsection{The expected marginal contribution}
\label{sec:exp_marg_contr}

% We are now going to formally introduce the expected marginal contribution of an individual under a given policy $\pol$. 
%As discussed before, we wish to make individually fair decisions while maximizing utility, where we identify the quality of individuals with their expected marginal contribution to the utility of the DM. 
The {\em marginal contribution} of an individual $i$ to a set $\act$ is given by $\util (\act + i) - \util (\act)$, where we mean by $\act + i$ that individual $i$ is being selected, i.e.\ $\act + i = (a_1, \dots, a_{i-1}, 1, a_{i+1}, \dots , a_N)$ for any $\act \in \Act$. In our case, we do not have a fixed set $\act$ by use of which we could compare marginal contributions of two individuals. We therefore define the {\em expected marginal contribution} (EMC) of an individual $i$ under a policy $\pol$ as
\begin{align}\label{eq:expected marginal contribution}
    \EMC_i \util(\pol, \bx) = \sum_{\act \in \Act} \pi(\act \mid \bx) \big[ \util(\act + i, \bx) - \util(\act , \bx) \big].
\end{align}
Informally, the EMC of individual $i$ corresponds to the gain (or loss) in expected utility when a policy is modified so as to always pick individual $i$.
\ifdefined \LongVersion
If we are given a distribution $\beta$ over populations, then we define the expected marginal contribution with respect to that distribution as
\begin{align*}
    \E_\beta [\EMC_j \util (\pol, \bx)] = \int_\bx \Delta_j \util (\pol, \bx) \beta(\bx).
\end{align*}
\fi
The concept of marginal contributions has been studied in cooperative game theory, where the celebrated Shapley value (\cite{shapley}) constitutes a fair resource allocation based on marginal contributions. The Shapley value is characterised by four axioms of fair division: efficiency, symmetry, linearity, and the treatment of null players. As we show below, the EMC satisfies analogous axioms, except for efficiency, which does not apply to the EMC as it lacks a corresponding normalisation.
\paragraph{Properties.}
The EMC satisfies the following axioms of fair division, where we omit $\bx$ for brevity.
\begin{enumerate}
    \item[1)] Symmetry: If $\util(\act + i) = \util(\act + j)$ for all $\act \in \Act$, then $\EMC_i \util (\pol) = \EMC_j \util (\pol) $ for all individuals $i, j \in \pop$ and policies $\pol \in \Pol$.
    \item[2)] Linearity: If $\util_1$ and $\util_2$ are two utility functions, then $\EMC_i (\alpha \util_1+ \beta \util_2) (\pol) = \alpha \Delta_i \util_1 (\pol) + \beta \Delta_i \util_2 ( \pol) $ for all individuals $i \in \pop$, policies $\pol \in \Pol$, and $\alpha, \beta \in \Reals$.
    \item[3)] Null player: If individual $i$ has zero contribution to every set, i.e.\ $\util(\act+i)=\util(\act)$ for all $\act \in \Act$, then $\EMC_i \util (\pol) = 0$ for all policies $\pol \in \Pol$.
\end{enumerate}


% These properties are - apart from {\em efficiency} which does not apply to the EMC - analogs to the axioms of fair division characterising the Shapley value. 
% In fact, we obtain the Shapley value when assuming an egalitarian policy. 

%\begin{lemma}
%Given a class of utility functions $\mathcal{U}$, the expected marginal contribution $\val_\pol$ is the only function of the expected %utility $\E_\pol \util$ up to linear scaling to satisfy the axioms of fair division given by 1.-3.
%\end{lemma}

%\begin{lemma}
%Given a class of utility functions $\mathcal{U}$, the expected marginal contribution $\val_\pol$ is the unique function up to linear %scaling to satisfy the axioms of fair division for every policy $\pol$.
%\end{lemma}

%\kbcomment{@Deba: Could you have a look into this Remark? I don't know how to put it.}
Furthermore, we obtain the Shapley value when assuming an egalitarian policy.
\begin{remark}\label{lemma:shapley egalitarian}
Under the egalitarian selection policy $\egpol(\act) = \frac{1}{(k+1) \binom{N}{k+1}}$ when $\| \act \|_1 = k$, the EMC $(\EMC_i \util (\egpol))_{1 \leq i \leq N}$ is equal to the Shapley value.
%expected marginal contribution of all the candidates $(\Delta_j U(\pol))_j$ are equal to their respective Shapley values. 
\end{remark}

%\begin{lemma}[Egalitarianism and Shapley Value]
%When the selection policy $\pol$ is egalitarian, i.e.\ $\frac{1}{(k+1){N\choose k+1}}$ for all the sets of cardinality $k$, expected marginal contribution of all the candidates $(\Delta_j U(\pol))_j$ are equal to their respective Shapley values. 
%\end{lemma}




%As a consequence, we observe by Lemma 1 and 2 that the (multinomial and softmax) policy gradient $\nabla_\theta \util (\pol_{\theta})$ %for multinomial or softmax policies 
%evaluated at $\pol_{\theta} = \egpol$ is equal to the Shapley value up to a constant factor.

%Using the expected marginal contribution to update our policy, our policy after each update will naturally deviate from the egalitarian policy as we increase meritocracy.


\subsection{Meritocracy and stability criteria}
\label{sec: meritocracy}
\tkbcom{Why 'other fairness criteria'?}
\mgcom{is "stability criteria" better? Or shall we just call it Meritocracy?}

% Utility maximisation is an obvious goal of the DM that intuitively clashes with fairness towards the individuals. However, we show that it is actually quite in line with meritocracy, when defining the merit of an individual as their contribution towards the utility. 

% Another desirable property for policies is that of smoothness which states that similar populations should lead to similar selection policies.

% \amgcomment{
% \textbf{Smoothness:}
% A policy $\pol$ is smooth, if $D(\pol(\act \mid \bx), \pol(\act \mid \bx')) \le \|\bx-\bx'\|$ for all $\act \in \Act$.
% }

% \amgcomment{TODO: What should the function $D$ look like?? }

% \amgcomment{In a sense, the notion of smoothness provides a fairness towards populations. If the population of college applicants this year, resembles the one from last year, it could be perceived as unfair if the selection policy drastically changes.}

With an estimation of the merit of individuals given by the EMC given a policy, we can define a meritocratic policy via the following two desirable properties. We omit $\bx$ for brevity in the following.

\begin{definition}[Swap stability]\label{definition:swap-stability}
A policy $\pol$ is called \emph{swap stable}\mgcom{swap-stable or swap stable?}, if for two individuals $i,j\in \pop$, from which $i$ is more likely to be selected, forcing $i$ to be selected and $j$ not to be selected yields a higher utility than vice versa. More formally, for any two individuals $i,j \in \pop$ with $\pol(i) > \pol(j)$ we have $\util(\pol+i-j) \ge \util(\pol-i+j)$, where $\util(\pol+i-j)=\sum_{\act \in \Act} \pol(\act)\util(\act+i-j)$.
\end{definition}
Note, that instead of writing $\util(\pol+i-j)$ we can also write $\util(\pol')$, where policy $\pol'$ shifts all the mass to sets that include $i$ but not $j$, i.e., $\pol'(a)= \pol(a)+\pol(a-i)+\pol(a+j)+\pol(a-i+j)$ if $a_i=1$ and $a_j=0$, and $\pol'(a)=0$ otherwise.
Thus swap stability guarantees that the utility of selecting $i$ but not $j$ is higher than the utility of selecting $j$ but not $i$ (under the shifted weights of $\pol$).
Analyzing this further, we can see that this is equivalent to $\EMC_i \util(\pol-i-j) \ge \EMC_j \util(\pol-i-j)$, where $\EMC_i \util(\pol-i-j)=\sum_{\act \in \Act} \pol(a)[U(a+i-j)-U(a-i-j)]= \util(\pol + i -j ) - \util ( \pol -i -j)$.
% =\sum_{\act \in \Act} \pol^+(a)(\util(\act+i)-\util(\act))$ and $\pol^+(a)= \pol(a)+\pol(a+i)+\pol(a+j)+\pol(a+i+j)$ if $a_i=a_j=0$, and $\pol'(a)=0$ otherwise, such that $\util(\pol-i-j)=\sum_{\act \in \Act} \pol^+(\act) \util(\act)$.\mgcom{We never actually defined what we mean by $\EMC_i \util(\pol-i-j)$. I guess we have $\EMC_i \util(\pol-i-j)=\sum_{\act \in \Act} \pol'(a)(\util(\act+i)-\util(\act))$. This is not very clear in the proof neither...}\tkbcom{Isn't it way easier to define $\util(\pol-i-j)$ via the utility and not a different policy?}

\begin{lemma}\label{lemma:swap-stability equivalence}
$\util(\pol+i-j) \ge \util(\pol-i+j)$ if and only if $\EMC_i \util(\pol-i-j) \ge \EMC_j \util(\pol-i-j)$
\end{lemma}

Hence, for a swap stable policy $i$'s merit, measured by expected marginal contribution when electing neither $i$ nor $j$, is higher than that of $j$ (under the shifted weights of $\pol$).


\begin{definition}[Local Stability]\label{definition:local-change-stability}
A policy $\pol$ is \emph{locally stable}, if for any $i \in \pop$ we have $\util(\pol) \ge \util(\pol+i)$, where $\util(\pol+i)=\sum_{\act \in \Act} \pol(\act)\util(\act+i)$.
\end{definition}
Instead of $\util(\pol+i)$ we can also write $\util(\pol'')$, where policy $\pol''$ shifts all the mass to sets that include $i$, i.e., $\pol'(a)= \pol(a)+\pol(a-i)$ if $a_i=1$, and $\pol''(a)=0$ otherwise.
Thus stability under local changes guarantees that the expected utility of selecting $i$ with certainty (under the shifted weights of $\pol$) is lower than the expected utility of $\pol$.
Further analysis shows that this is equivalent to $\EMC_i \util(\pol) \le 0$.
% Thus a policy that is locally stable is also locally optimal.

\begin{lemma}\label{lemma:local-change-stability equivalence}
$\util(\pol) \ge \util(\pol+i)$ if and only if \mgcom{implies?}$\EMC_i \util(\pol) \le 0$.\tkbcom{99\% sure that it is an equivalence.}
\end{lemma}

\begin{definition}[Meritocracy]
A policy $\pol$ is called \emph{meritocratic}, if it is swap-stable and locally stable.
\end{definition}
This notion of meritocracy ensures that our policy is fair to individuals, in the sense that individuals with lower chances of being selected have no justification of increasing their chances or swapping their chances of being selected with another individual given a meritocratic policy.
Thus, meritocratic policies also satisfy some degree of local optimality in terms of utility. In fact, 
 a policy that selects a utility maximising set, or a local optimum of the utility function, is swap stable and stable under local changes, and thus meritocratic. However, when considering additional constraints on the policies,
%  e.g., by restricting the number of individuals that may be selected or including some diversity constraints, 
always selecting the utility optimal set may not be feasible. In this case, the notion of meritocracy provides some guidance of which feasible policy is fair and should be selected.
 Note, that the egalitarian policy,
%  that assigns every set (and thus every individual) the same probability, 
while being far from utility maximising, is also not necessarily meritocratic. 
%  Also, the utility of this policy might be far from optimal.
 
\begin{example}%[\cref{ex: shapley} continued]
Consider a college admission setting with applicants Alice (A), Bob (B), Carlos (C), and David (D) with utilities as 
%in \cref{ex: shapley} 
presented in the following table.
% , where columns represent applicant sets $\act \in \Act$.
\begin{center}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
        A & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 \\
        B & 0 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 0 & 1 & 1 \\
        C & 0 & 0 & 0 & 0 & 1 & 1 & 1 & 1 & 0 & 0 & 0 & 0 & 1 & 1 & 1 & 1 \\
        D & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\\hline
        Utility 
          & 0 & 1 & 0 & 0 & 1 & 1 & 0 & 2 & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 0
    \end{tabular}
\end{center}

% The utility maximising set if clearly $\{A,B,C\}$ with a utility of 2. 
Policy $\pi_{max}(\act)$, that selects the utility maximising set $\{A,B,C\}$ with probability $1$,
is meritocratic. 

The egalitarian policy $\pi_{eg}$ that assigns every subset of applicants probability $1/16$ is not stable under local changes and thus not meritocratic since $\util(\pi_{eg})=9/16$ but $\util(\pi_{eg} + A)=6/8$. 
Because all applicants have equal selection probabilities the statement of swap-stability vacuously holds for $\pi_{eg}$. 

Now consider the policy $\pol$ that selects the sets $\{A,B,C\}, \{B,C,D\}, \{A,B,C,D\}$ with probability $1/3$ each (and all other sets w. p. 0). $\pol$ is stable under local changes, since $\util(\pol)=2/3$ whereas $\util(\pol+A)=\util(\pol+B)=\util(\pol+C)=2/3$ and $\util(\pol+D)=0$. However, $\pol$ is not swap stable, since $B$ is selected w.p. $1$ and $A$ w.p. $2/3$, but $\util(\pol-B+A)=1$ and $\util(\pol+B-A)=0$.
\end{example}


\begin{lemma}\label{lemma:determinstic_optimal_meritocractic}
Any deterministic policy $\pi$ maximising utility, i.e.\ $\pi \in \argmax_{\pi} \util(\pi, \bx)$, is meritocratic. 
\end{lemma}
Note that this is in general not true for optimal {\em stochastic} policies, which we elaborate upon in the proof of aforementioned lemma in the supplemental material. 

==> sections/List_of_changes.tex <==
\section{List of Changes}

This paper was previously peer reviewed at FORC 2021. Based on the suggestions of the reviewers we made the following adjustment: We extended the related work section. We also included examples to underline the rational behind our modelling choice and make the paper more reader friendly, and give more motivation and a formal definition for meritocracy, and a new measure to quantify the deviation from meritocracy. Here, we also clarified the relation between meritocracy and the EMC. As the utility functions under consideration are not limited to model social welfare of the population, we cut all mentions of social welfare. In our experiments, we include fairness constraints in our experiments that are separate from the original utility. Previously some other fairness constraints were included directly in the utility function. We also cut out a deeper comparison of our work with that of Kearns et al. 2017 because of the significant differences in the settings and space limitations. Furthermore, we do not discuss the scenario anymore, where only a distribution over populations is given.


==> sections/abstract.tex <==
Typically, merit is defined with respect to some intrinsic measure of
worth. We instead consider a setting where an individual's worth is
\emph{relative}: when a Decision Maker (DM) selects a set of
individuals from a population to maximise expected utility, it is
natural to consider the \emph{Expected Marginal Contribution} (EMC) of
each person to the utility. We show that this notion satisfies an
axiomatic definition of fairness for this setting. We also show that
for certain policy structures, this notion of fairness is aligned with
maximising expected utility, while for linear utility functions it is
identical to the Shapley value. However, for certain natural policies,
such as those that select individuals with a specific set of
attributes (e.g. high enough test scores for college admissions),
there is a trade-off between meritocracy and utility maximisation.  We
analyse the effect of constraints on the policy on both utility and
fairness in an extensive experiments based on college admissions and
outcomes in Norwegian universities.
    
  

==> sections/ack.tex <==
Many thank you to Rachel Cao, Yang Liu, David Parkes and Goran Radanovic for long discussions about fairness in the set selection setting that partly served to inspire this line of work. We would also like to thank Mauricio Byrd for contributing to early validation experiments.

==> sections/experiments_old.tex <==
\section{REMOVE: Old Experimental Section}
\label{sec:experiments}
In this section, we perform an empirical case-study on the set selection of individuals in a college admission system to test different algorithms with regards to achieved utility and our notion of meritocracy. The goal of the experiments is primarily to analyse the effect of different policy structures and secondarily to demonstrate that utility maximisation is sufficient for promoting group fairness notions (e.g.\ diversity or statistical parity). 

\subsection{Data and Experimental Setup}
\paragraph{Data generation.} 
Data is generated through simulation. From this, we first generate records for $4,000$ students, which represent the admitted students to the faculty from previous years. Each student is represented by a feature vector including a high school GPA for three specific fields (e.g.\ humanities or science), gender and high school. We assume that students come from $10$ different schools and that the school to some extent depends on the individual's ethnicity (being majority, large minority, or small minority). In addition, each student is provided with a graduation result (numerical between $0$ and $1$), which we use to train a prediction model.
The graduation grade is based on two latent variables: 1) talent: an innate quality, normally distributed across the population, and 2) skill: based on talent, but can be developed or hindered. Skill development is affected by school quality and societal gender biases. For evaluation, we generate another $500$ students from the simulator from who we wish to select a subset. A detailed description of the simulator is given in the Appendix~\ref{app:simulator}.

\paragraph{Modelling graduation using regression.} 
As we wish to estimate the success for each student, we train a linear regression model on the data $D$ from the $4,000$ students to predict the graduation results of the students observed in the decision phase. We refer to these predictions as {\em predicted outcomes}. The trained predictor $\mathbf{f}$ takes the data $\bx$ of students from this year as input and predicts the outcome $y_i \in [0,1]$ of the $i$-th individual: $\mathbf{f}(i) \defn \Pr (y_i \mid \bx, D)$.


\paragraph{Algorithms for set selection.}
We examine the behaviour of separable linear and threshold policies. For threshold policies, we use the high school GPA as a numerical three dimensional feature and add the gender and school as one-hot encoded categorical features. For both policy structures, we allow the policy gradient algorithms $250$ updates to converge. In addition, we consider uniform set selection as a trivial lower baseline and for a robust benchmark, implement stochastic greedy set selection (see e.g.\ \cite{qian2018approximation}) which essentially performs dynamic ranking of individuals according to marginal contributions.

Even though we believe that ranking is not particularly suitable for this problem, we can use {\em predicted outcomes} of an individual to rank them. We implement the cross-population noisy-rank algorithm of \cite{kearns2017meritocratic}, which produces a probabilistic ordering over the population based on individuals' relative percentiles. 
In its original form, the noisy-rank algorithm requires us to only select an individual $i$ if all higher ranked individuals are being selected as well. To combine this with a utility function,  we select individuals in the order induced by the ranking until an individual has negative contribution. We will refer to this in our experiments as {\em noisy-rank}.
%We also want relax the fairness notion of (\citet{kearns2017meritocratic}) so that individuals are being {\em considered} in the order of the ranking but individuals can be skipped if their contribution is negative without  terminating the selection process. We refer to this as {\em greedy-rank}.  \cdcomment{However, this does not guarantee that higher ranked individuals will be selected first, so what's the point?}


\subsection{Designing utility functions}
\label{sec:utility}

From a utilitarian social-welfare point of view, the DM is interested in the {\em outcomes} of her decisions. This requires having a utility function that depends on the actual outcomes - in the university scenario, for instance the graduation result encoded in some numerical value. In addition, the DM might have a cost associated with the selection of a student, so that it might only be favourable for the DM to select a student, if the gain in utility from adding the student to the set exceeds the cost $c$ of selecting her. In case of {\em linear utility}, the DM's utility function $u : \Act \times \CY \to \Reals$ then takes form
\begin{align*}
    u(\act, \by) = \sum_{i \in \act} y_i - c \cdot |\act|,
\end{align*}
where we slightly abuse notion when writing $i \in \act$ to mean that $i$ is being selected under decision $\act$, i.e.\ $i \in \{ k : a_k = 1\}$.

The DM might also be interested in promoting {\em diversity} in the study body, e.g.\ by admitting candidates from different backgrounds or demographics. For instance, the DM may wish to admit approximately the same number of female and male students. In our case, we can define group types, $\mathcal{T} = \{\text{gender}, \text{schools}\}$, and groups of such type, e.g.\ $\mathcal{G}_{\text{gender}} = \{\text{male}, \text{female}\}$. This allows us to define utilities accounting for the demographic background of applicants. A natural choice for a diversity promoting utility is the {\em log-linear utility over groups}:
\begin{align*}
    u (\act, \by) = \sum_{T \in \mathcal{T}} \sum_{G \in \mathcal{G}_T} \log \Big(\sum_{i \in \act \cap G}  y_i \Big) - c \cdot |\act|
\end{align*}
as it naturally promotes egalitarian selection among groups.


\iflongversion
%\paragraph{Log-linear utility over groups.} % Diminishing return utility.
%A natural choice for a diversity promoting utility is the log-linear utility
%\begin{align*}
%    u (\act, \mathcal{X}) = \sum_{T \in \mathcal{T}} \sum_{G \in \mathcal{G}_T} \log \Big(\sum_{i \in \act \cap G}  y_i \Big)
%\end{align*}
%as it naturally promotes egalitarian selection among groups. 
While this can be a good choice with respect to a group feature such as gender since it promotes a 50/50 distribution, it might be desirable for the DM to have a utility that takes group sizes into account.

\paragraph{Weighted log-linear utility over groups.}
We consider a modification of the log-linear utility function representing the goal of having a student body that demographically represents the application pool. Here, the cumulative outcome of a group is multiplied by a function that is maximal when the probability of selecting an individual of a group is close to the ratio of that group in the total application pool. More precisely, we define the weighted log-linear utility
\begin{align*}
    u (\act, \mathcal{X}) =  \sum_{T \in \mathcal{T}} \sum_{G \in \mathcal{G}_T} \log \Big( f_{r_G} (p_G) \sum_{i \in \act \cap G}  y_i \Big) ,
\end{align*}
where $r_G = \frac{|G|}{N}$ denotes the ratio of group $G$ w.r.t.\ the total application pool, and $p_G = \frac{|\act \cap G|}{|\act|}$ the empirical probability of selecting an individual from group $G$. The function $f_{r_G}(x)$ can be any function centered around $r_G$ that is increasing for $x \leq r_G$ and decreasing for $x \geq r_G$, e.g.\ $f_{r_G}(x) = 1 - |x-r_G|$.


In practice, we do not have access to the actual outcomes $\mathbf{y}$ of individuals and therefore use the trained predictor $\mathbf{f}$ to estimate the utility of a set by $\util(\act, \bx) = \E_{\mathbf{y} \sim \mathbf{f}} [u (\act, \by)]$ (cf.\ Section \ref{sec:setting}). %denoted $\util(\act, \bx)$ before.

%Here, outcomes $y_i$ of the protected group $S$ are increased by a factor of 1.5 if the probability $p_S$ of selecting an individual from group $S$ is not less than delta away from the ratio of the protected group to the total applicant pool. We define (WE CHANGE THIS INTO SOMETHING DIFFERENT PROMOTING LOW STATISTICAL PARITY)
%\begin{align*}
%    u (A, \mathcal{X}) = \sum_{i \in A} y_i + \ind{p_S \in [r_S - \delta, r_S + \delta]} \gamma \sum_{i \in A \cap S} y_i,
%\end{align*}
%where $\gamma$ is a ... factor. Such a utility function may compensate for bias in the model (?).

%the diminishing returns utility to the type of group. Such tuning can be accomplished by defining preferences such as $p_{\text{science}} = 0.5$, $p_{\text{arts}} = 0.3$, etc. and using the preference-based log-linear utility
%\begin{align*}
%    u (A, \mathcal{X}) = \E_{\mathbf{y} \sim \mathbf{f}} \left[  \sum_{T \in \mathcal{T}} \sum_{G \in \mathcal{G}_T} p_G \log \Big(\sum_{i \in A \cap G}  y_i \Big) \right]
%\end{align*}
\fi

\notesfalse
\ifnotes
\textbf{A diminishing returns utility based on outcomes only.} If the utility should only be a function of the outcomes and NOT of group defining attributes, then we could define the following return diminishing utility functions:
\begin{align*}
    u(\act, y) = \sum_{j=1}^m \Big( d_j \sum_{i \in \act} y_{i, j} \Big)^{\frac{1}{2}},
\end{align*}
where $m$ is the number of groups, e.g.\ fields of study, and $d_j$ is the approximate number of students we want to select with successful outcomes in that group, e.g.\ graduating in that field of study. (or if we want to select exactly $k$ individuals use $d_j \cdot k$ so that $d_j$ denotes the approx.\ percentage of students we wish to select from group $j$) 

If we want to promote diversity along more than a single axis, we can consider the utility
\begin{align*}
    u(A, y) = \sum_{s=1}^t \sum_{j=1}^m \Big( d_{m,j} \sum_{i \in A} y_{i, j} \Big)^{\frac{1}{2}},
\end{align*}
where $t$ denotes the number of criteria along which we define groups.

\textbf{A diminishing returns utility based on group affiliations.} 
Let $T$ denote the set containing the type of groups present in the population, e.g.\ $T = \{\text{gender}, \text{ethnicity}, \text{field of study}\}$. Let $\mathcal{G}_t$ denote the groups of type $t$, e.g.\ $\mathcal{G}_{\text{gender}} = \{ \text{male}, \text{female}\}$, and $G_{j}$ the individuals that are members in group $j$, e.g.\ $G_{\text{male}} = \{1, 4, 9, \dots\}$. We define the utility
\begin{align*}
    u(A, y) = \sum_{t\in T} \sum_{j \in \mathcal{G}_t} \Big( d_{t,j} \sum_{i \in A \cap G_j} y_i \Big)^{\frac{1}{2}},
\end{align*}
where $d_{t,j}$ denotes the approximate number that we wish to select from group $j$ of type $t$. For instance, we may aim for 50\% male and female admissions and therefore define $d_{\text{gender}, \text{male}} = 0.5$. ($A \subset \{1, \dots, N\}$)
\fi



%\kbcomment{Maybe drop this completely.}
%We assume that we do not have access to the latent variable talent, but only observe the high school GPA of student that it depends on the talent as well as the school the student is coming from. 
%However, it is appealing to view the talent as a ground truth quality or worth of a student. We then want to measure to what degree our decisions correspond to the talent of individuals. For this reason, we measure the Spearman's rank correlation of the talent and the final policy.


%Note that we interpret a positive expected marginal contribution under policy $\pol$ as what the DM would gain under his current policy from always picking an individual. It is important to note the difference between the expected marginal contribution and the policy gradient as calculated for instance in Lemma \ref{lemma:multinomial gradient}. The difference lies in the fact that the policy gradient is oblivious to the share an individual is already receiving under the current policy. Therefore, if $\pol(1) = 1$ the expected marginal contribution is zero, whereas the policy gradient may still be nonzero. It therefore seems more intuitive to use the expected marginal contribution rather than the residual gradient as a measure of unfairness. In addition, this has the advantage that we have a universal measure of unfairness that can be used to compare different approaches. 



\iffalse
\subsection{Measuring diversity}


In ecology, economics, and political science, quantifying diversity in form an index is studied historically~\cite{simpson1949measurement,hill1973diversity,laakso1979effective,jost2006entropy,chao2016phylogenetic}. In general, if individuals are chosen from $C$ communities (or groups) according to some demographic feature, the \textit{expected diversity} of order $l \in \Reals^+$ is defined as
\begin{equation*}\label{eqn:diversity}
    \diversity_l \triangleq \left( \sum_{i=1}^C p_i^l \right)^{1/(1-l)},
\end{equation*}
where $p_i$ is the probability of selecting an individual from the $i$-th community. These are called Hill numbers in ecology~\cite{hill1973diversity}. Here, we use diversity of order $l=2$, which is also called the inverse Simpson's index~\cite{simpson1949measurement}, where higher values of $\diversity_l$ represent higher diversity. This specific quantification of diversity is used to represent the effective number of parties in an election process~\cite{laakso1979effective} or to represent the effective number of different species in an ecosystem~\cite{chao2016phylogenetic}. We adopt this well studied diversity measure to quantify the expected number of groups 
%(e.g.\ gender, ethnicity) 
having representatives in the selected set of individuals. As we have different types of groups in our situation, we take the sum of $\diversity_2$ over all group types (i.e.\ gender, school).
 

%In addition, we want to consider the bias in our decision making. To this end, we define {\em statistical parity} as 
%\begin{align*}
%    \max_{G, \tilde{G} \in \mathcal{G}} \vert \P (\text{selecting } i \mid i \in G) - \P(\text{selecting } i \mid i \in \tilde{G}) |
%\end{align*}
%Thus, if we try and optimise a policy for maximising this diversity measure, it allows us to ensure fairness and to select as diverse set as possible.

\fi

\subsection{Performance analysis}
We report the results of the experiments for linear and log-linear utility in Tables~\ref{tab:linear_utility} and~\ref{tab:log_linear_utility} ,respectively. The experiments are conducted with a population of $500$ students, and a selection cost per individual of $0.5$ and $0.2$ for linear and log-linear utility, respectively. We evaluate the algorithms according to the {\em true} outcomes of individuals generated by the simulator which are unavailable to the algorithms. 

\input{sections/table_results}


From Tables \ref{tab:linear_utility} and \ref{tab:log_linear_utility}, we observe that closeness to optimal expected utility corresponds to low residual EMCs. The residuals for the separable linear policy and the stochastic greedy algorithm are non-zero due to prediction errors of the trained model. With respect to the predicted outcomes, both algorithms achieve almost zero residuals for both utility types (cf. further results in Tables~\ref{tab:linear_utility_detail} and~\ref{tab:loglinear_utility_detail} in Appendix~\ref{app:tables}). Thus, the residuals of the separable linear policy and the greedy algorithm can be seen as a deviation from meritocracy caused by the DM's imperfect predictions.

%We observe that the linear separable policy and stochastic greedy algorithm achieve highest utility for both, linear and log-linear utility.

The threshold policy remains highly unstable as we do not project the policy to the next closest vertex in the simplex, which results in relatively low utility and high residuals. The aim of a threshold policy is to provide simple criteria for admission as these are attractive from the point of view of transparency and explainability. In order to guarantee such clarity and explainability, we want our policy to make decisions about individuals in the original feature space without mapping to higher dimensions. As a result, the threshold policy struggles whenever individuals are in the optimal set (i.e.\ have positive contribution), but are surrounded by sub-optimal individuals with similar features. 
%Figure~\ref{fig:threshold linear selection comparison} illustrates this for a simplified situation with $100$ students and $2$ features.
This is visualised in Figure \ref{fig:threshold linear selection comparison}, where we conducted the experiments with a simplified simulator having only two grade features (apart from gender and school) for illustrative purposes.

Tables~\ref{tab:linear_utility} and~\ref{tab:log_linear_utility} show that meritocratic fairness notion of~\cite{kearns2017meritocratic} is too restrictive in our setting as selection is stopped too early. Consequently, the residual EMCs are even higher than for the uniform policy as the majority of the population could have positively contributed but were not considered. The comparison between noisy-rank and the uniform selection also yields the observation that while close to optimal utility generally implies low residual EMCs, low utility does not necessarily imply high residuals. For instance, the policy that is selecting the whole population always achieves zero residuals while achieving low utility in general.


%When allowing the algorithm to skip individuals in its selection, the ranking gives an optimal set for linear utility. In the case of log-linear utility, the ranking approaches struggles as it selects individuals successively and individually and thus, cannot account for synergies in the population effectively.

When comparing the inverse Simpson indices $\diversity_2$ for both utilities, we see that the log-linear utility successfully increases the diversity in the selected set compared to the linear utility. Here, the stochastic greedy algorithm and the separable linear policy achieve almost maximal diversity of $12$, i.e. when every group has the same probability of selection. 
%Rewrite?
This is representative of the possibilities when using utility maximisation as a framework for group fair set selection as we could clearly design utilities promoting other group fairness notions such as statistical parity.
In particular, when applying the log-linear utility and choosing students according to their marginal contribution we encode their demographic background implicitly into their ``merit". This approach of utility design to promote affirmative actions is may be more appealing to the DM than designing different admission criteria for different groups. 
%which leads to similar approaches as cross-population ranking \citep{kearns2017meritocratic}.


\begin{figure}[h]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{graphs/feature_space/lin_utility_threshold_illustration.pdf}
  \caption{Linear utility}
  \label{fig:linear utility}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{graphs/feature_space/log_utility_threshold_illustration.pdf}
  \caption{Log-linear utility}
  \label{fig:log-linear utility}
\end{subfigure}
\caption{The selection of the separable linear policy (red circles) and the soft decision boundary $\vparam^T \bx$ determined by the threshold policy (blue line) illustrated in the feature space of $100$ students generated with two numerical grade features (x-axis and y-axis) as well as gender and school. Each circle represents a student by means of her feature vector. Every student above the line has $>0.5$ probability of selection under the threshold policy.}
\label{fig:threshold linear selection comparison}
\end{figure}

% Making decisions according to a threshold policy that constitutes admission criteria brings the advantage that decisions/policies can be made transparent and are easily explainable. However, from Tables \ref{tab:linear_utility} and \ref{tab:log_linear_utility} we see that such policies may fail to be meritocratic with respect to EMCs. We illustrate this in Figure \ref{fig:threshold linear selection comparison}, where we use a simplified model with only two features that - apart from a latent unobservable variable talent - determine the final outcome of a student. 
%We then plot the discriminant function $\vparam^T\bx$ calculated by the threshold policy as well as indicate the selection of the linear separable policy that chooses individuals meritocratic according to EMCs. 
% Figure \ref{fig:threshold linear selection comparison} also lays out the difficulties that can arise when the DM wishes to treat similar individuals (in terms of features) similarly while maximizing utility. The separable linear policy that is may reject an individual and select another individual with high probability even though both individuals have almost identical grades (more generally features).



==> sections/introduction2.tex <==

\section{Introduction}
\label{sec:introduction}

Machine learning is now pervasively used to assist high-stake
decision making, with significant consequences for individuals and
organisations. 
We are especially interested in the case where the
decision maker (DM) must fix a policy to select a \emph{set} of individuals from a
population so as to maximise expected utility, where the utility function over sets \tkbcom{This is weird. We either have a utility function over sets or a non-linear utility, right? What is non-linear over sets?} may be non-linear. %, without having individual scores. Thus, the DM cannot use a naive solution of ranking individuals. 
Finding a utility maximising policy can be complemented by additional constraints, e.g., diversity constraints.
%For instance, according to  \cite{diaz2013gender}, if we wish to maximise innovative ideas, we would prefer teams with gender diversity. 
Furthermore\tkbcom{The following is irrelevant for our work, isn't it?}, the DM's utility function may not only represent their narrow self interests but also some notion of social welfare. This means that a policy
maximising utility would be fair in terms of its aggregate benefit to
society. In fact, it is possible to define a utility function that partly takes into account notions of group fairness, such as egalitarianism.
% We can also assume that expected utility represents an appropriate notion of social welfare. 

In addition to maximising utility, the DM may also like their selection policy to be meritocratic. 
The obvious question that arises is how to define meritocracy for general utility functions over candidate sets and what the relationship between utility maximisation and meritocracy is. 

%In this paper, we suggest using a notion of \emph{expected individual contribution} to the utility to measure the merit of individuals. We define meritocracy as rewarding the individuals with more utility contribution the most and we show that for certain policy structures, maximising utility also achieves meritocracy. 
In the following, we motivate our notion of meritocracy by discussing different fairness considerations underlined with examples.

{\em Egalitarianism} is a notion of fairness where individuals' chances
of obtaining a reward are independent of personal characteristics. In
the simplest case, we wish our decisions to be independent of
\emph{any} personal characteristics, which is achievable through a uniformly random lottery. More typically, we wish our
decisions to be independent of
sensitive characteristics such as gender or ethnicity. 

\begin{example}\label{ex: egalitarian-policy}
Alice (female, average grade: B), Bob (male, average grade: D),    Carlos (male, average grade: A)  and  David (male, average grade: B) apply to college. An egalitarian policy assigns equal probabilities of admission to all candidate sets, and thus to all applicants independent of features.
\end{example}

An egalitarian policy is not always good choice. In our example, it could be unfair to give everyone equal admission chances, when Bob's estimated chances of actually succeeding in his studies are low, while Carlos may have good chances of succeeding. 

{\em Meritocracy} suggests that individuals with higher ``worth'' obtain higher rewards, i.e. higher selection probability. As long as there is an inherent, static measure
of worth this is a well-defined notion. In our setting this is true in particular if the DM obtains a utility $u_i$ for selecting candidate $i$, with the total utility being the sum of individual utilities. Then for any $i,j$ such that $u_i>u_j$, corresponding rewards $r_i, r_j$ to the two candidates should obey $r_i > r_j$.
\begin{example}\label{ex: meritocracy-for known merits}
  If the DM's utility is equal to the number of people that graduate, then the unique worth of an individual is equal to their probability of graduation. If Alice has a utility (e.g., success chance) of $0.5$, Bob $0.2$, Carlos $0.9$, and David $0.7$, then their reward, i.e. probabilities of being admitted to college, should follow the order $r_{Carlos} > r_{David} > r_{Alice} > r_{Bob}$.
\end{example}

However, in many settings,
including ours, worth is relative and dependent on circumstances. In
particular,  the relative contribution of an individual
to utility depends on who else has been selected (and more generally
the DM's policy). % so that it is a constantly shifting quantity.
Let us now extent the above example to illustrate this problem.

\begin{example}\label{ex: shapley}
  In another scenario Alice (A), Bob (B), Carlos (C) and David (D) may be candidates for an engineering team. Then overall utility we can extract from the team is not a simple linear function, as the multi-faceted qualities of the individuals interact. For example, B works well only when both A and B are there, but not D, otherwise he is disruptive. W can model this by setting $u(X)=0$ when Bob is among the selected set $X$, except for $u(\{A,B,C\})=2$. In all other cases the utility is $1$, except for $u(\emptyset)=0$. 
\end{example}

\cdcom{I am a bit confused about this example. If we have a fixed team, then the Shapley value suggests a renumeration to give.} 
The well known Shapley value $S(i)=\sum_{X\subseteq \mathcal{N}\setminus\{i\}} \frac{|X|!(|\mathcal{N}|-|X|-1)!}{|\mathcal{N}|!} \cdot (u(X\cup \{i\})-u(X))$ computes the marginal contribution of $i$ to the utility over sets of candidates.
We have: $S(Alice) = 14/12$, $S(Bob)=-5/12$, $S(Carlos) = 14/12$, $S(David)=-6/12$. 
Basing the selection policy on the Shapley values of students is meritocratic and arguably fair, as the Shapley value satisfies desirable properties, see \cite{shapley}.
However, if a selection policy is given in advance, we may want to weight the possible selection sets by their probability. If a set is not likely to be selected, e.g., because it is known that sets including Bob most often lead to low utility, then the contribution of a candidate to this set should not weight as much. We estimate the merit of an individual, given a selection policy, by these re-weighted contributions to utility which we call \emph{expected marginal contributions}. 
% If, e.g.,  maximal 3 candidates can be admitted, a feasible policy would set the probability of selecting all candidates to $0$, such that David's (negative) contribution to the set \{Alice, Bob, Carlos\} should not be counted.
% In our work we estimate the worth or merit of an individual by their expected marginal contribution.
We then define a policy to be meritocratic, when forcing an individual $j$ to be selected within this policy, or to be selected by removing another individual $i$ with higher probability, is not beneficial in terms of utility. This definition can be reinterpreted to match the merit of an individual given by expected marginal contributions.


\paragraph{Contribution.}
We define a notion of meritocracy for policies in set selection problems and arbitrary utility functions relating to individual
\emph{expected marginal contributions} (EMC). This is analogous to marginal utilities for a basket of goods in economics, which must
necessarily depend on both the \emph{population} under consideration
and the DM's \emph{policy} for selection. It contrasts works
on set selection based on ranking, which implicitly define meritocracy
through a static worth for every individual.  In particular, when
the DM's policy is egalitarian, the EMC is identical to the Shapley value\amgcomment{, see} \cite{shapley}. A
natural way to shift the policy towards meritocracy would then be to
increase the probability of selecting individuals proportionally to
their EMC. If we apply this algorithmic idea to any initial DM policy,
we show that we arrive at a \emph{policy gradient algorithm} for
policies that are separably parameterised over the population.
%where the DM is free to choose any subset from the population. 
For these, maximising utility also achieves meritocracy,
as the gradient is a linear transformation of the EMC\mgcom{is this still true?}.  For other
policies, e.g.\ those relying on a threshold, this does not hold and
meritocratic outcomes cannot be guaranteed when maximising
utility. Then, we can measure the deviation from meritocracy in terms of the residual EMC. Experimentally, we analyse different policy structures in a college admission setting and illustrate the relation of meritocracy with respect to EMCs to policy structures and utility maximisation.
We experimentally instantiate the policy gradient framework on linear and log-linear utility, and separable linear and threshold policies. Here, we also add contraints that guarantee statistical parity\mgcom{is that true?}. We measure the expected utility and diversity\mgcom{do we still measure diversity?} of the solution to quantify the solution quality. We show that separable policies achieve expected utility, residual EMC, and diversity index that are close to optimal, whereas policies based on thresholding and ranking are significantly sub-optimal\mgcom{check if this is still true after running experiments}\mgcom{also say something about the deviation from meritocracy which, as I understand it, is the main goal of the experiments}. 


==> sections/table_200_50.tex <==
\begin{table*}[t!]
\begin{minipage}{0.48\textwidth}
%\begin{table}
\centering
\caption{{\em Linear utility:} From 200 select 50.}\label{tab:diverse_5_10}
\scalebox{1}{
\begin{tabular}{l|c|c|c} 
\toprule
\begin{tabular}[c]{@{}c@{}}Algorithm\\\end{tabular} & $U$ & $Res$ &  $Div$ \\ 
\hline
Softmax      & \textcolor{red}{41.40}      & \textcolor{red}{61.39}                     & 4.24       \\ 
\hline
Linear                       & 29.14     & 73.47                     & 4.47       \\ 
\hline
Greedy                     & \textcolor{red}{41.24}    & \textcolor{red}{61.55}                     & 4.23       \\
\hline
Uniform                    & 25.68      & 79.18                     & \textcolor{red}{4.51}       \\ 
\bottomrule
\end{tabular}}
\end{minipage}\hfill
\begin{minipage}{0.48\textwidth}
\centering
\caption{{\em Log-linear utility:} From 200 select 50.}\label{tab:util_5_10}
\scalebox{1}{
\begin{tabular}{l|c|c|c} 
\toprule
\begin{tabular}[c]{@{}c@{}}Algorithm\\\end{tabular} & $U$ &  $Res$ &  $Div$ \\ 
\hline
Softmax   & 26.80      &  25.56     & \textcolor{red}{12.48}      \\ 
\hline
Linear      & 23.67   &  29.31     & 11.18       \\ 
\hline
Greedy      & \textcolor{red}{27.49}     &  \textcolor{red}{18.89}      &  11.51      \\
\hline
Uniform      & 22.36      & 32.51      & 10.87   \\ 
\bottomrule
\end{tabular}}
%\end{table}
\end{minipage}\vspace*{-1.2em}
\end{table*}

==> sections/table_500_200.tex <==
Preliminary results from experiments:
\begin{table*}[t!]
\begin{minipage}{0.48\textwidth}
%\begin{table}
\centering
\caption{{\em Linear utility:} Utility , residual and diversity when selecting 200 students from 500.}\label{tab:diverse_5_10}
\scalebox{1}{
\begin{tabular}{l|c|c|c} 
\toprule
\begin{tabular}[c]{@{}c@{}}Algorithm\\\end{tabular} & $U$ & $Res/U$ &  $Div$ \\ 
\hline
Softmax                                           & 152.15      & 0.46                     & \textcolor{red}{11.62}       \\ 
\hline
EMC-Softmax                                      & 153.58      & 0.45                     & 11.48       \\ 
\hline
Linear                                            & 122.23     & 0.57                     & 11.55       \\ 
\hline
Stoch.\ Greedy                                  & \textcolor{red}{154.13}      & 0.45                     & 11.49       \\
\hline
Greedy                                            & 153.69     & 0.45                     & 11.48       \\ 
\hline
Uniform                                           & 112.93      & NaN                     & 11.53       \\ 
\bottomrule
\end{tabular}}
\end{minipage}\hfill
\begin{minipage}{0.48\textwidth}
\centering
\caption{{\em Log-linear utility:} Utility , residual and diversity when selecting 200 students from 500.}\label{tab:util_5_10}
\scalebox{1}{
\begin{tabular}{l|c|c|c} 
\toprule
\begin{tabular}[c]{@{}c@{}}Algorithm\\\end{tabular} & $U$ &  $Res/ U$ &  $Div$ \\ 
\hline
Softmax  & 46.27      &  0.25   &   13.46    \\ 
\hline
EMC-Softmax   & 46.36      &  0.24     & \textcolor{red}{13.74}      \\ 
\hline
Linear      & 43.35   &  0.31     & 12.28       \\ 
\hline
Stoch.\ Greedy      & \textcolor{red}{46.91}     &  \textcolor{red}{0.20}     &  13.69      \\
\hline
Greedy      & 45.60     &  0.22     &  11.48      \\
\hline
Uniform      & 41.42      & NaN     & 11.63   \\ 
\bottomrule
\end{tabular}}
%\end{table}
\end{minipage}\vspace*{-1.2em}
\end{table*}


==> sections/table_results.tex <==

\iflongversion
\begin{table*}[h]
\begin{minipage}{0.48\textwidth}
%\begin{table}
\centering
\caption{{\em Linear utility:} Achieved utility ($U$), residual EMCs ($Res$), correlation between latent variable talent and probability of selection ($Corr$), and inverse Simpson's index ($Div$).}\label{tab:diverse_5_10}
\scalebox{1}{
\begin{tabular}{l|c|c|c|c} 
\toprule
\begin{tabular}[c]{@{}c@{}} Algorithm \\\end{tabular} & $U$ & $Res$ & $Corr$ & $Div$ \\ 
\hline
Linear                                            & 0      & 0                     & 0       \\ 
\hline
Threshold                                           & 0      & 0                     & 0       \\ 
\hline
Greedy                                  & 0     & 0                     & 0       \\ 
\hline
%Greedy-rank                                            & 0      & 0                     & 0       \\
%\hline
Noisy-rank                                    & 0      & 0                     & 0       \\
\hline
Uniform                         & 0      & 0                     & 0       \\
\bottomrule
\end{tabular}}
\end{minipage}\hfill
\begin{minipage}{0.48\textwidth}
\centering
\caption{{\em Log-linear utility: Achieved utility ($U$), residual EMCs ($Res$), correlation between latent variable talent and probability of selection ($Corr$), and inverse Simpson's index ($Div$).} }\label{tab:util_5_10}
\scalebox{1}{
\begin{tabular}{l|c|c|c|c} 
\toprule
\begin{tabular}[c]{@{}c@{}} Algorithm \\\end{tabular} & $U$ & $Res$ & $Corr$ & $Div$ \\ 
\hline
Linear                                            & 0      & 0                     & 0       \\ 
\hline
Threshold                                           & 0      & 0                     & 0       \\ 
\hline
Greedy                                  & 0     & 0                     & 0       \\ 
\hline
%Greedy-rank                                            & 0      & 0                     & 0       \\
%\hline
Noisy-rank                                    & 0      & 0                     & 0       \\
\hline
Uniform                         & 0      & 0                     & 0       \\
\bottomrule
\end{tabular}}
%\end{table}
\end{minipage}\vspace*{-1.2em}
\end{table*}

\else
%for short version
\begin{table*}[h]
\begin{minipage}{0.48\textwidth}
%\begin{table}
\centering
\caption{Expected utility and residual EMCs w.r.t.\ actual outcomes for {\em linear utility} ($c=0.5$), as well as inverse Simpson's index.}\label{tab:linear_utility}
\scalebox{1}{
\begin{tabular}{l|c|c|c} 
\toprule
\begin{tabular}[c]{@{}c@{}} Algorithm \\\end{tabular} & $\,\,\util(\pol)\,\,$ & $\res(\pol)$ & $\diversity_2$ \\ 
\hline
Linear &24.53  & 2.00  & 10.01  \\ 
\hline
Threshold & 13.03 & 8.83 & 10.00      \\ 
\hline
Greedy  & 25.07 & 1.62 & 10.14 \\ 
\hline
Noisy-rank & 1.25 & 26.80 &  6.47 \\
\hline
%Greedy-rank & 25.10 & 1.62 & 10    \\
%\hline
Uniform & -4.10 & 14.10 & 10.65   \\
\bottomrule
\end{tabular}}
\end{minipage}\hfill
\begin{minipage}{0.48\textwidth}
\centering
\caption{Expected utility and residual EMCs w.r.t.\ actual outcomes for {\em log-linear utility} ($c=0.2$), as well as inverse Simpson's index.}
\label{tab:log_linear_utility}
\scalebox{1}{
\begin{tabular}{l|c|c|c} 
\toprule
\begin{tabular}[c]{@{}c@{}} Algorithm \\\end{tabular} & $\,\,\util(\pol)\,\,$ & $\res(\pol)$ & $\diversity_2$ \\ 
\hline
Linear & 16.64 & 0.59 & 11.42    \\ 
\hline
Threshold & 12.34 & 1.69 & 10.24       \\ 
\hline
Greedy & 17.03 & 0.06 & 11.73 \\ 
\hline
%Greedy-rank & 15.96 & 0 & 11.72 \\
%\hline
Noisy-rank & 11.83 & 37.04 & 9.75    \\
\hline
Uniform & 7.63 & 8.91  & 10.71  \\
\bottomrule
\end{tabular}}
%\end{table}
\end{minipage}%\vspace*{-1.2em}
\end{table*}
\fi
